Quantization of Generative Adversarial Networks for Efficient Inference: a Methodological Study

Generative adversarial networks (GANs) have an enormous potential impact on digital content creation, e.g., photo-realistic digital avatars, semantic content editing, and quality enhancement of speech and images. However, the performance of modern GANs comes together with massive amounts of computations performed during the inference and high energy consumption. That complicates, or even makes impossible, their deployment on edge devices. The problem can be reduced with quantization -- a neural network compression technique that facilitates hardware-friendly inference by replacing floating-point computations with low-bit integer ones. While quantization is well established for discriminative models, the performance of modern quantization techniques in application to GANs remains unclear. GANs generate content of a more complex structure than discriminative models, and thus quantization of GANs is significantly more challenging. To tackle this problem, we perform an extensive experimental study of state-of-art quantization techniques on three diverse GAN architectures, namely StyleGAN, Self-Attention GAN, and CycleGAN. As a result, we discovered practical recipes that allowed us to successfully quantize these models for inference with 4/8-bit weights and 8-bit activations while preserving the quality of the original full-precision models.

==> GAN quantization arxiv (1)/acknowledgments.tex <==
%\documentclass[aa.tex]{subfiles}

\begin{document}
This work was supported by Samsung Research. We also thank Egor Zakharov for helpful comments.
\end{document}

==> GAN quantization arxiv (1)/conclusion.tex <==
%\documentclass[aa.tex]{subfiles}

\begin{document}

In this work, we have conducted an extensive experimental study of state-of-art quantization techniques' effectiveness to uniform quantization of generative adversarial networks. The study concerns post-training quantization and quantization-aware training techniques applied to generators of three diverse GAN architectures, namely style-based GAN, self-attention GAN, and cycle-consistent GAN. The results suggest that these models can be successfully quantized for 4/8-bit inference with negligible quality degradation. We hope that the results of this paper will set up a starting point for future research on the quantization of GANs and allow using GANs in a lot of new AI-driven products.
%With this being said, future work should pay more attention to quantization of generative models (especially to post-training quantization), as this task is generally more challenging than quantization of discriminative models and may benefit from specialized approaches. 

\end{document}

==> GAN quantization arxiv (1)/contribution.tex <==
%\documentclass[aa.tex]{subfiles}

\begin{document}


\end{document}

==> GAN quantization arxiv (1)/discussion.tex <==
%\documentclass[aa.tex]{subfiles}

\begin{document}


The results of experiments demonstrate that GANs \underline{can be} successfully quantized for fixed-point inference with negligible quality degradation (see Figure \ref{fig:sample}).
In particular, we show that \emph{learned step size quantization} provides a recipe for the successful quantization of generative adversarial networks. We find this approach to generalize across the most important GAN architectures, specifically StyleGAN, SAGAN, and CycleGAN.

Interestingly, we reveal that, in contrast to classification models, GANs cannot be quantized with modern methods of post-training quantization and require more resource-demanding methods of quantization-aware training. 
The results also shed light on what technical details matter for successful GAN quantization. 
For instance, we show that using quantiles instead of minimal and maximal values for tuning quantization intervals is crucial for well-performing post-training quantization and moving average-based quantization-aware training. 
In accordance with prior work \cite{krishnamoorthi2018quantizing}, we show that per-channel quantization does not provide significant benefits when using quantization-aware training.  


\end{document}

==> GAN quantization arxiv (1)/experiments.tex <==
%\documentclass[aa.tex]{subfiles}


\begin{document}


This section presents experimental results of quantization techniques efficiency assessment for the three GAN models under consideration. We use horse2zebra \cite{zhu2017unpaired}, CelebA \cite{liu2015faceattributes}, and FFHQ (thumbnails 128x128) \cite{karras2019style} datasets to train CycleGAN, SAGAN, and StyleGAN models, respectively. Our experiments are based on the PyTorch quantization module \cite{NEURIPS2019_9015}. We will make the code and checkpoints publicly available. 

It is important to note that in addition to the standard practice of using Frechet inception distance (FID) \cite{heusel2017gans} for comparison of generated images with real ones, we utilize FID to directly measure similarity between images generated by the quantized model and images generated by the full-precision model (using the same latent codes). We found this metric, which we refer to as qFID, to be a more informative reconstruction quality measure.

\subsection{Post-training quantization}


Vanilla post-training quantization considered in this work is based on observation of quantiles of weights' and activations' distributions. Specifically, we tune the quantization ranges by a moving average of observed quantiles during the generation of 500 images (one by one), with moving average momentum being equal to 0.99. We examine 1.0/0.0, 0.9999/0.0001, 0.999/0.001, 0.99/0.01 pairs of quantiles for upper and lower quantization range bounds, respectively, and observe significant dependency of quality of generated images on quantiles' values for activations (see Figure \ref{fig:quantiles}). In contrast, no significant improvements were observed during tuning quantiles for weights. Based on our experiments, we find pairs of quantiles 0.9999/0.0001 to be optimal for post-training quantization of activations for StyleGAN and CycleGAN, whereas pair 1.0/0.0 is optimal for SAGAN. For weights' quantization, we observe the pair of quantiles 0.9999/0.0001 to perform slightly better than other tested configurations and use it throughout our experiments.

In addition to vanilla post-training quantization, we explore advanced PTQ techniques described in \ref{ptq} for style-based generator architecture. We consider styled convolutional blocks as blocks for the reconstruction of synthesis network and pairs of linear layer and subsequent nonlinearity (leaky ReLU) for the reconstruction of mapping network (see \cite{karras2019style} for definition mapping and synthesis networks).  
%As it was mentioned in \ref{ptq} we employ two strategies for learning weight quantization, namely adaptive rounding (AdaRound, AR) \cite{nagel2020up} and straight-through estimator (STE) with learned step sizes \cite{esser2019learned}. 
The results of the experiments are summarized in Table \ref{table:ptq}. For both strategies, we use a training sample of size 896 images and batch size of 16 images; we refer the reader to the Appendix \ref{app:impl} for other implementation details. An interesting finding of this work is that STE-based BRECQ significantly outperforms AdaRound-based BRECQ for 8-bit quantization while being inferior for 4-bit quantization. Furthermore, AR-BRECQ provides better FID for 4-bit weights quantization than for 8-bit. We attribute this counterintuitive result to the nature of adaptive rounding, which by design allows only for local optimization of rounding rule. Thus, the 4-bit adaptive rounding may have richer space for optimization than the 8-bit one due to larger quantization step sizes. Overall, the results suggest that post-training quantization may provide samples of reasonable quality (see Figure \ref{fig:sample}); however, to go further, quantization-aware training is needed.


\begin{table}[!h]
  \caption{Performance (FID and qFID, lower is better) of post-training quantization techniques in application to quantization of style-based generator. }   \label{table:ptq}
    \vskip 0.15in
 \begin{center}
   \begin{tabular}{|l|c|>{\centering\arraybackslash}p{1.8cm}>{\centering\arraybackslash}p{1.8cm}|>{\centering\arraybackslash}p{1.8cm}>{\centering\arraybackslash}p{1.8cm}|}
 \hline %   \toprule
    \multirow{2}{*}{Method} & \multirow{2}{*}{Per-channel}  &
      \multicolumn{2}{c|}{Number of bits per weight: 8} &
       \multicolumn{2}{c|}{Number of bits per weight: 4}  \\
      & & {FID ($\downarrow$)} & {qFID ($\downarrow$)} & {FID ($\downarrow$)} & {qFID ($\downarrow$)}  \\
      \hline
    full-precision & - & 26.3 & 0.0  & 26.3 & 0.0   \\ \hline
     \multirow{2}{*}{vanilla PTQ} & \checkmark & 66.5  & 51.2 & 73.1 & 60.3  \\
     & $\times$  & 65.9 & 50.4 & 73.5 & 62.4  \\ \hline
      
     \multirow{2}{*}{AR-BRECQ} & \checkmark  & 66.8 & 49.9  & \textbf{61.2} & \textbf{46.2} \\
     & $\times$ & 65.1 & 48.4 & 61.9 & 48.1  \\ \hline
    
    STE-BRECQ  & $\times$ &  \textbf{51.7} & \textbf{35.9} & 61.7 & 51.6  \\

    \hline
  \end{tabular}
   \end{center}

\end{table}


%\begin{figure}%
%    \begin{center}
%    \subfigure[\centering Vanilla %PTQ]{{\includegraphics[width=6cm]{images/quantile%s_ptq.pdf} }}%
%    \qquad
%    \subfigure[\centering MA-QAT (a8/w8, %per-channel)]{{\includegraphics[width=6cm]{images%/quantiles_qat.pdf} }}%
%    \end{center}
%    \caption{Dependency of StyleGAN qFID on %quantile corresponding to the upper bound of quantized activations range (the lower bound quantile is chosen symmetrically). }%
 %   \label{fig:quantiles}%
%\end{figure}

\begin{figure}%
    \centering
    \subfloat[\centering Vanilla PTQ]{{\includegraphics[width=7.5cm]{images/quantiles_ptq.pdf} }}%
    \qquad
    \subfloat[\centering MA-QAT (a8/w8, per-channel)]{{\includegraphics[width=7.5cm]{images/quantiles_qat.pdf} }}%
    \caption{Dependency of StyleGAN qFID on quantile corresponding to the upper bound of quantized activations range (the lower bound quantile is chosen symmetrically). }%
    \label{fig:quantiles}%
\end{figure}

\begin{figure}[h!]
\begin{center}
\centerline{\includegraphics[width=1.0\columnwidth]{images/stylegan_pics.pdf}}
\caption{Sample images along with Frechet inception distance scores~(lower is better, $\cdot$ \textcolor{gray}{/} $\cdot$ correspond to 4\textcolor{gray}{/}8-bit weights respectively) for  various quantization methods applied to StyleGAN generator. 
Vanilla PTQ with quantiles-based statistics matching (quantile) generates significantly better samples than baseline (min-max).
In general, quantization-aware training~(highlighted by \textcolor{caribbeangreen}{green}) produces significantly more realistic samples than post-training quantization~(highlighted by \textcolor{bluebell}{blue}). 
The learned step size quantization with quantile initialization~(LSQ-QAT) allows quantization with negligible quality degradation. Activations are quantized to 8 bit, weights are quantized per-tensor with the number of bits outlined at the top of the figure. Note that for the generation of these images we have used the truncation trick to avoid sampling from extreme regions \cite{karras2019style}.}
\label{fig:sample}
\end{center}
\end{figure}


\subsection{Quantization-aware training}



As described in \ref{qat}, for quantization-aware training, we use a sum of adversarial and perceptual losses. Thus, the resulting loss function has three additive components, namely adversarial loss, perceptual content loss, and perceptual style loss. Each term's relative weights are tuned via the grid search over 27 parameter combinations to optimize performance on the SAGAN quantization. The search space is a cartesian product of the following sets $\{0, 0.01, 0.1\}$ (adversarial loss), $\{1, 3, 10\}$ (content loss) and $\{10^4, 3 \cdot 10^4, 10^5\}$ (style loss). We did not find huge deviations in the results depending on the combination used. However, one combination performed slightly better than others, that is $0.01$ coefficient for adversarial loss, $3$ for content loss, and $3 \cdot 10^4$ for style loss. Given that these parameters did not account for a significant impact on the performance, we did not re-run the grid search for other concerned GAN models and used this set of parameters for all quantization-aware training experiments. Besides, we studied the importance of the considered distillation objective by replacing it with pixel-wise mean squared error (MSE). Overall, the perceptual loss significantly outperformed the MSE loss for the concerned models; please refer to the Appendix \ref{app:obj} for detailed results.



%The relative performance of LSQ-based and Moving Average-based procedures for tuning quantization parameters appear to depend on the particular GAN model. LSQ-based approach considerably outperforms MA-QAT for Self-Attention Generative Adversarial Network. In contrast, MA-QAT with properly selected quantiles for quantization of activations has superior performance for Cycle-consistent Generative Adversarial Network (see Table \ref{48bit_table}). Furthermore, the LSQ-QAT and MA-QAT approaches provide similar quality of Style-based GAN quantization. The optimal quantiles for MA-QAT also depend on a particular GAN model and do not necessarily coincide with those selected at the post-training quantization stage (see Figure \ref{fig:quantiles}). We found pairs 0.999/0.001, 0.9999/0.0001, and 0.9999/0.0001 to give optimal performance for StyleGAN, SAGAN, and Cycle-GAN respectively, please refer to Appendix \ref{app:impl} for other hyperparameters and implementation details.
The LSQ-based procedure for tuning quantization parameters appears to outperform the moving average-based one considerably (see Table \ref{Tab:48bit_table}). This effect is especially noticeable in the case of 4-bit quantization of weights. It is noteworthy that we found it beneficial for the CycleGAN model to perform 50 initial training epochs using the MA-QAT procedure while applying the LSQ-based one during the subsequent 50 epochs. Besides, the optimal quantiles for MA-QAT depend on a particular GAN model and do not necessarily coincide with those selected at the post-training quantization stage (see Figure \ref{fig:quantiles}). We found the pairs 0.999/0.001, 0.9999/0.0001, and 0.999/0.001 to give optimal performance for StyleGAN, SAGAN, and Cycle-GAN, respectively.
%, please refer to Appendix \ref{app:impl} for other hyperparameters and implementation details.

\begin{table}[!h]
  \caption{Performance of quantization-aware training techniques. MA-QAT and LSQ-QAT denote moving average and learned step size strategies for tuning quantization parameters. “wxay” means x-bit weights
and y-bit activations. $^*$: LSQ is applied only during the last 50 epochs.} \label{48bit_table} 
    \vskip 0.15in
 \centering
  \begin{tabular}{|l|c|c|>{\centering\arraybackslash}p{1.3cm}>{\centering\arraybackslash}p{1.3cm}|>{\centering\arraybackslash}p{1.3cm}>{\centering\arraybackslash}p{1.3cm}|>{\centering\arraybackslash}p{1.3cm}>{\centering\arraybackslash}p{1.3cm}|}
 \hline %   \toprule
     \multirow{2}{*}{Method} & \multirow{2}{*}{Per-channel} & \multirow{2}{*}{Bits}  &
      \multicolumn{2}{c|}{CycleGAN} &
       \multicolumn{2}{c|}{SAGAN} &
     \multicolumn{2}{c|}{StyleGAN}  \\
      & & & {FID ($\downarrow$)} & {qFID ($\downarrow$)} & {FID ($\downarrow$)} & {qFID ($\downarrow$)} & {FID ($\downarrow$)} & {qFID ($\downarrow$)} \\
      \hline
    full-precision & - & - & 62.4 & 0.0 & 138.6  & 0.0 & 26.3 & 0.0 \\ \hline
     \multirow{4}{*}{vanilla PTQ} & \checkmark & a8/w8  & 98.8  & 71.9 & 139.6 & 81.1 & 66.5 & 51.2 \\
     & $\times$ & a8/w8  & 103.0 & 74.5 & 145.3 & 86.8 & 65.9 & 50.4 \\
     & \checkmark & a8/w4  & 118.3 &  85.1 & 265.4 & 287.2 & 73.1 & 60.3 \\
     &  $\times$ &  a8/w4 & 154.0  & 115.5 & 309.4 & 325.2 & 73.5 & 62.4 \\ \hline

      
     \multirow{4}{*}{MA-QAT} & \checkmark & a8/w8  & 63.7 & 38.3  & 125.9 & 10.4 & 32.3 & 14.3 \\
     & $\times$ & a8/w8  & \textbf{63.1} & 40.8 & \textbf{124.8} & 11.9 & 32.6 & 14.7 \\
     & \checkmark & a8/w4  & \textbf{69.3} & 50.7 & \textbf{114.2} & 29.1  & 40.1 & 23.3 \\
     &  $\times$ &  a8/w4  & 112.5 & 88.3 & 128.7 & 31.5 & 37.2 & 18.5 \\ \hline
      
    % \multirow{4}{*}{LSQ-QAT } & \checkmark & a8/w8  & 64.4 & 36.4 & 130.0 & 5.5 & 32.8 & 12.6 \\
    
   \multirow{2}{*}{LSQ-QAT }  & $\times$ & a8/w8  & \textbf{63.1}$^*$ & \textbf{36.1}$^{*}$ & 130.1 & \textbf{5.6} & \textbf{28.8} & \textbf{8.5} \\
   %  & \checkmark & a8/w4  & 67.7 & 42.8 & 130.0 & 8.7 & 36.0 & 14.5 \\
     &  $\times$ &  a8/w4  & 71.4$^{*}$ & \textbf{47.6}$^{*}$ & 125.8 & \textbf{9.0} & \textbf{33.1} & \textbf{11.0}\\ 

    \hline
  \end{tabular}

 \label{Tab:48bit_table}
\end{table}



\end{document}

==> GAN quantization arxiv (1)/intro.tex <==
%\documentclass[aa.tex]{subfiles}

\begin{document}

Generative adversarial networks (GANs) are the tool of choice for a variety of computer vision tasks involving generative modeling \cite{karras2019style, zhang2017beyond, zhu2017unpaired}. However, the expressiveness of modern deep neural networks comes along with tremendous computational and memory resources spent during the inference phase, with GANs being a clear illustration of this tendency \cite{brock2018large}. This circumstance significantly complicates the deployment of such models in real-world applications, especially on edge devices, where memory and latency are of the main concern. 

Over the past few years, considerable research attention has been dedicated to the compression of deep neural networks. The most popular compression techniques include pruning \cite{he2017channel, molchanov2017variational}, efficient architecture design \cite{chollet2017xception, howard2017mobilenets}, knowledge distillation \cite{hinton2015distilling, chen2017learning}, and quantization \cite{krishnamoorthi2018quantizing, yao2020hawqv3}. The last one is of particular research attention due to several reasons. First, it is “orthogonal” to the majority of other compression techniques, meaning that quantization can be applied to an already architecturally compressed and pruned model.
%Second, quantization is very effective in terms of quality degradation versus compression degree relation, for instance, it was shown that 8-bit quantization of deep classification models leads to 4x model size reduction and speedups inference phase up to 3 times, while maintaining the accuracy of the original full-precision model \cite{yao2020hawqv3, esser2019learned}.
Second, the energy consumption of quantized models is decreased significantly due to reduced data movement \cite{krishnamoorthi2018quantizing}. And lastly, quantization facilitates the deployment of neural networks on FPU-free devices, as it enables integer-only inference \cite{yao2020hawqv3}.

Most of the relevant works explore quantization techniques in the context of image classification, whereas quantization of generative models is considered as a more challenging and understudied task \cite{wan2020deep}. In this paper, we reduce the concerned research gap by extensively studying the applicability of different quantization methods to generative adversarial networks. The key contributions of this work are as follows:
\begin{enumerate}
%\item We reviewed the recently emerged quantization techniques for both discriminative and generative models and analyze their adequacy to practical GAN quantization.
\item We explore the effectiveness of state-of-art post-training quantization techniques for quantization of style-based generative adversarial network. 
\item We carry out an experimental study of quantization-aware training techniques in application to three diverse GAN architectures, namely self-attention GAN \cite{zhang2019self}, cycle-consistent GAN \cite{zhu2017unpaired} and style-based GAN \cite{karras2019style}, and for the first time report successful 4-bit quantization of these models.
\item To the best of our knowledge, this is a pioneering work primarily dedicated to uniform quantization of different types of generative adversarial networks, providing a valuable starting point for future research. 
\end{enumerate}

\end{document}

==> GAN quantization arxiv (1)/method.tex <==
%\documentclass[aa.tex]{subfiles}

\begin{document}
In this section, we provide a description of experimental design choices and motivate them.


\subsection{Uniform and non-uniform quantization}

Generally, two types of quantization are distinguished in a principled way, namely uniform and non-uniform quantization. The first one maps values of weights and activations to a uniform grid of fixed-point representations:
\begin{equation} \label{eq:symquant}
    x_q = \Delta \cdot \mathrm{clamp}\big(\mathrm{round}(\frac{x}{\Delta}), t_{\min}, t_{\max} \big) = \Delta \cdot x_{int},
\end{equation}
where $x$ denotes a full precision real-valued number, $x_q$ is the corresponding quantized value, $\Delta$ is a quantization step size (a parameter to be determined during quantization process), $x_{int}$ is an integer representation, $\mathrm{clamp}(x, t_{\min}, t_{\max})$ denotes clamping $x$ to the $[t_{\min}, t_{\max}]$ interval. By replacing floating-point tensors with uniformly quantized ones, it becomes possible to perform typical calculations (e.g., convolution) in low bitwidth integer arithmetic, thus reducing computational resources. In contrast, non-uniform quantization maps values to a non-equidistant grid of quantized values, thereby being more flexible \cite{zhang2018lq, park2018value}.  However, these approaches are harder to be deployed on hardware, since the execution of low bitwidth operations is not as straightforward as for integer arithmetic in the uniform quantization case. Hence, we consider uniform quantization only.

\subsection{Static and dynamic quantization}

Since the distribution of activations may vary significantly depending on the model input, it is desirable to adapt quantization of activations dynamically during inference. Dynamic quantization does this by recomputing quantization parameters for each batch of data independently. Although dynamic quantization allows for a flexible approximation of activations, it induces considerable overhead in computations. In contrast, static quantization uses precomputed quantization parameters for activations, thus being more computationally efficient. With this being said, we decided to use static quantization to achieve maximal efficiency.

\subsection{Per-chanel and per-tensor weight quantization}

Another important concept is per-channel quantization of weights \cite{krishnamoorthi2018quantizing}. Per-channel quantization assigns distinct parameters (quantization scales) to each convolutional kernel, enabling flexible quantization of weights. At the same time, it does not involve significant overhead in computations. Nevertheless, considerable research efforts were concentrated on eliminating the need for per-channel quantization of weights to simplify the implementation of quantized operations \cite{nagel2019data, nagel2020up}. In our work, we investigate the importance of per-channel quantization for GANs.

\subsection{Symmetric and asymmetric quantization}
The concept of asymmetric (affine) quantization relates to the usage of flexible zero-points in the quantization scheme. Specifically, one can modify the formula \eqref{eq:symquant} in the following way:
\begin{equation} \label{eq:asymquant}
    x_q = \Delta \cdot \bigg ( \mathrm{clamp}\big(\mathrm{round}(\frac{x}{\Delta} + z), t_{\min}, t_{\max} \big) - z \bigg ) = \Delta \cdot (x_{int} - z),
\end{equation}
where $z$ is an integer corresponding to zero point. Hence, asymmetric quantization allows modeling non-zero-centered distributions of weights and activations more effectively. However, it introduces additional computational cost, which is negligible for asymmetric quantization of activations but might be significant in asymmetric quantization of weights \cite{krishnamoorthi2018quantizing}. Thus, for our experiments we use symmetric signed ($t_{\min} = -2^{n-1}$, $t_{\max} = 2^{n-1} - 1$, where $n$ is the number of bits) quantization for weights and asymmetric for activations.


\subsection{Post-training quantization} \label{ptq}


We consider two approaches to post-training quantization of GANs. The first one is based on observation of statistical functions and later referred to as vanilla PTQ. In this approach, we propose to tune quantization parameters so that the minimal and maximal quantized values are matched to the certain quantiles of full-precision values distribution. The optimal quantiles for weights and activations are determined independently and shared between all layers. Despite the simplicity of this approach, we found it to provide significant improvements over naive baseline, which matches minimal and maximal quantized values to minimum and maximum of full-precision values.

%The second approach to post-training quantization of GANs is built upon recent work of \cite{li2021brecq}. Similarly to this technique, we block-wisely optimize weights and quantizers by matching activations' feature maps to the ones of the full-precision model. We consider two quantization learning methods. The first one (STE-BRECQ) relies on {straight-through estimator}, and {learned step size quantization} (LSQ) \cite{esser2019learned} for differentiation through rounding operation. The second method (AR-BRECQ) employs {adaptive rounding} technique for weights quantization and applies LSQ only for learning quantization of activations (likewise \cite{li2021brecq}).

Another approach to post-training quantization of GANs is built upon recent works \cite{li2021brecq, esser2019learned, nagel2020up}. Consider a generator model $f$ composed of $n$ sequential blocks $f = f_n \circ  f_{n - 1} \circ \dots \circ f_1$ and its quantized version $f^{q} = f^q_n \circ  f^q_{n - 1} \circ \dots \circ f^q_1$. Let us denote the input and output of the $n$-th full-precision block as $X_n$ and $Y_n$, respectively. Similarly to BRECQ technique \cite{li2021brecq}, we block-wisely optimize weights and quantizers by matching activations' feature maps to the ones of the full-precision model:
\begin{equation} \label{eq:local}
    (\{\Delta_k, z_k\}_k, \{W^q_l\}_l) = \argmin \limits_{\{\Delta_k, z_k\}_k, \{W_l^q\}_l} \| f^q_i(X_{i}) - Y_i \|_F^2,
\end{equation}
where $\{\Delta_k, z_k\}_k$ are the quantization parameters for activations and possibly weights within $f^q_i$, $\{W^q_l\}_l$ are the quantized weights of $f^q_i$. We consider two quantization learning methods. The first one (STE-BRECQ) relies on {straight-through estimator} (STE) \cite{krishnamoorthi2018quantizing} and learned step size quantization (LSQ) \cite{esser2019learned} for differentiation through rounding operation. The second method (AR-BRECQ) employs {adaptive rounding} technique for weights quantization and applies LSQ only for learning quantization of activations (as in \cite{li2021brecq}). We also tried to incorporate squared gradient information into the loss function \eqref{eq:local} as it was proposed in \cite{li2021brecq}, but did not observe any improvements.

\subsection{Quantization-aware training} \label{qat}

Although post-training quantization is fast and requires a small data sample, its performance is restricted by limited resources. Hence, we make use of quantization-aware training to further reduce the quality degradation associated with quantization. Similarly to \cite{wang2020gan}, we employ a sum of adversarial and reconstruction losses for quantization-aware training:

\begin{equation}\label{perceptual}
    L(\phi_q, \theta) = L_{adv} + \beta \cdot L_{rec} = \mathbb{E}_{x \sim \mathrm{inp}} \bigg [ V_{\mathrm{LSGAN}} \big (D(f_q(x; \phi_q); \theta), D(f(x; \phi); \theta) \big ) + \beta \cdot d \big (f_q(x; \phi_q ), f(x; \phi) \big ) \bigg ],
\end{equation}
where $V_{\mathrm{LSGAN}}$ is the least squares GAN loss \cite{mao2017least}, $D(\cdot; \theta)$ denotes the discriminator with its parameters $\theta$, $f(\cdot;\phi)$ and $f_q(\cdot; \phi_q)$ are the full-precision generator and its quantized version, respectively, $d$ denotes the perceptual reconstruction loss \cite{johnson2016perceptual}, $\beta$ is the reconstruction weight hyperparameter. We follow the common practice of using straight-through estimator (STE) \cite{krishnamoorthi2018quantizing} for weights fine-tuning and study two strategies for tuning of quantization parameters. In the first one (MA-QAT), quantization parameters are adjusted by observing statistics of full-precision values during training. Specifically, similarly to vanilla PTQ, the ranges of quantized values are defined by moving averages of observed quantiles.
%We empirically select optimal pair among 0.99/0.01, 0.999/0.001, 0.9999/0.0001, and 1.0/0.0 to quantize activations and fix the pair to 0.9999/0.0001 for weights. 
The quantization parameters are adjusted by such a procedure during the first 50 epochs and remain fixed during subsequent epochs. Another strategy is based on learned step size quantization \cite{esser2019learned} with learnable zero points\footnote{Our implementation is based on codes from PyTorch quantization module (\href{https://github.com/pytorch/pytorch/blob/382781221de4fd3c8035285ce803efb757b5c104/torch/quantization/_learnable_fake_quantize.py}{link}).}. For both strategies, the quantization parameters are initialized using quantiles-based post-training quantization. In addition,  we tried to fix quantization parameters before quantization-aware training, following \cite{wang2020gan}. However, it appeared to be considerably worse than the strategies mentioned above.



\end{document}

==> GAN quantization arxiv (1)/related.tex <==
%\documentclass[aa.tex]{subfiles}

\begin{document}

\subsection{Quantization methods}

Quantization of neural networks is a popular compression technique that is based on the replacement of accurate floating-point operations by less accurate low-bit quantized operations. There have been significant advances in the quantization of deep classification models recently. The emerged methods can be roughly divided into post-training quantization (PTQ) and quantization-aware training (QAT) categories. Post-training quantization aims to quantize neural networks using a small part of the dataset (in some cases no data at all) for calibration of quantization parameters to ensure a certain local criterion (e.g., correspondence of minimum and maximum, MSE minimality). Recent work \cite{nagel2020up} showed that
minimizing the mean squared error (MSE) introduced in
the preactivations might be considered (under certain assumptions) as the best possible local criterion and performed optimization of rounding policy based on it. Works \cite{hubara2020improving} and \cite{wang2020towards} utilize the same local criterion but optimize weights and quantization parameters directly and employ per-channel weight quantization, thus considering a simplified task. BRECQ technique \cite{li2021brecq} further generalizes this idea by utilizing improved local objective enhanced with squared gradient information and taking advantage of block-wise granularity of the neural networks. In our experiments with PTQ, we use a similar approach, minimizing the MSE introduced in activations at the block-level granularity. Although post-training quantization of discriminative models has shown significant promise, it is still inferior to quantization-aware training, a technique that tunes model parameters directly on the task of interest using stochastic gradient descent. Despite QAT was originally used for weights fine-tuning only, recent works \cite{esser2019learned, jain2019trained} proposed to learn quantization parameters jointly with weights. The concerned methods employ the straight-through estimator (STE) technique to effectively differentiate through rounding operation, providing the state-of-art quantization quality.  The performance of the most noticeable PTQ and QAT techniques is summarized in Tables \ref{table_pqt} and \ref{table_qat}, respectively. In our work, we make use of the arguably most effective QAT technique, namely learned step size (LSQ \cite{esser2019learned}).



\begin{table}[h!]
\caption{Post-training quantization techniques. The table demonstrates ImageNet top1 accuracies for different architectures (RN -- ResNet, MBv2 -- MobileNetv2). The signed numbers in brackets $(\cdot)$ shows difference with the corresponding full-precision baseline reported in the paper. “wxay” means x-bit weights 
and y-bit activations.} \label{table_pqt}
\vskip 0.15in
\begin{center}
 \begin{tabular}{|>{\centering\arraybackslash}p{1.5cm}|>{\centering\arraybackslash}p{2cm}|>{\centering\arraybackslash}p{1.2cm}|>{\centering\arraybackslash}p{1.2cm}|>{\centering\arraybackslash}p{1.2cm}|>{\centering\arraybackslash}p{1.2cm}|}
\hline
  \multirow{2}{*}{Method} & \multirow{2}{*}{Per-channel}  & RN18 (a8/w8) & MBv2 (a8/w8) &  RN18 (a4/w4) &  RN50 (a4/w4) \\ 
  \hline
     Baseline \cite{krishnamoorthi2018quantizing} & \multirow{2}{*}{$\times$} & $69.2$ ($-0.5$)   & $0.1$ ($-71.8$) & \multirow{2}{*}{$-$} & \multirow{2}{*}{$-$}  \\ \hline
      Baseline \cite{krishnamoorthi2018quantizing} & \multirow{2}{*}{$\checkmark$} &  $69.7$ ($-0.1$)  & $69.7$ ($-2.2$) & \multirow{2}{*}{$-$} & \multirow{2}{*}{$-$}\\ \hline
   AdaRound \cite{nagel2020up} & \multirow{2}{*}{$\times$} &  $69.7$ ($+0$)  & $71.2$ ($-0.5$) & \multirow{2}{*}{$-$} & \multirow{2}{*}{$-$}\\ \hline
      CalibTIB \cite{hubara2020improving} & \multirow{2}{*}{$\checkmark$} & \multirow{2}{*}{$-$} & $73.0$ ($+0$) & $69.4$ ($-2.6$)  & $75.1$ $(-2.1)$ \\ \hline
    Bit-Split \cite{wang2020towards} & \multirow{2}{*}{$\checkmark$} & $69.7$ ($+0$) &  \multirow{2}{*}{$-$} & $67.5$ ($-2.1$) & $73.7$ ($-2.4$) \\ \hline 
    BRECQ \cite{li2021brecq} & \multirow{2}{*}{$\times$} & $71.0$ ($-0.1$)  & $72.4$ ($-0.1$) & $69.6$ ($-1.5$)  & $75.1$ ($-1.9$) \\ \hline     
\end{tabular}

\end{center}
\end{table}

  

\begin{table}[h!]
  \caption{Quatization-aware training techniques.  The table demonstrates ImageNet top1 accuracies for different architectures. Notations follow the table \ref{table_pqt} .} \label{table_qat}
  \vskip 0.15in
\begin{center}
    
 \begin{tabular}{|>{\centering\arraybackslash}p{1.5cm}|>{\centering\arraybackslash}p{2cm}|>{\centering\arraybackslash}p{1.2cm}|>{\centering\arraybackslash}p{1.5cm}|>{\centering\arraybackslash}p{1.2cm}|>{\centering\arraybackslash}p{1.2cm}|}
\hline
 \multirow{2}{*}{Method} & \multirow{2}{*}{Per-channel} & RN50 (a8/w8) & RN50 (a8/w4) & MBv2 (a8/w8) &  RN18 (a4/w4) \\ 
  \hline
    Baseline \cite{krishnamoorthi2018quantizing} & \multirow{2}{*}{$\checkmark$} & 75.0 ($-0.6$) & 73.0 ($-2.6$) & $70.9$ ($-1.0$) & \multirow{2}{*}{$-$} \\ \hline 
    \multirow{3}{*}{LSQ \cite{esser2019learned}} & \multirow{3}{*}{$\times$} & $76.8$ ($-0.1$) & $76.7$ ($-0.2$)  \textbf{a4/w4}  & \multirow{3}{*}{$-$} & $71.1$ ($+0.6$) \\ \hline 
    \multirow{2}{*}{TQT \cite{jain2019trained}} & $\times$  & $75.4$ ($+0$) & $74.4$ ($-1.0$)  & $71.8$ ($-0.1$) & \multirow{2}{*}{$-$} \\ \hline 
\end{tabular}

\end{center}
\end{table}

\subsection{Generative Adversarial Networks}

Originating from \cite{goodfellow2014generative}, generative adversarial networks have undergone numerous modifications and improvements over the past few years \cite{arjovsky2017wasserstein, gulrajani2017improved, zhang2019self, zhu2017unpaired, karras2019style}. In this paper, we focus on quantization of three architecturally distinct variants of GANs, which are CycleGAN \cite{zhu2017unpaired}, SAGAN \cite{zhang2019self} and StyleGAN \cite{karras2019style}. CycleGAN model tackles unpaired image-to-image translation problem by imposing cycle-consistency on the training process. From an architectural point of view, the generator of this model is a fully convolutional neural network with residual blocks. In contrast, the generator of SAGAN is augmented with self-attention layers in order to facilitate long-range dependency modeling. 
%Although self-attention blocks were proven to be effective and are widely used in other works \cite{brock2018large}, we observed that these blocks account for the largest quantization errors among all SAGAN layers, thus being challenging to quantize.
Another important type of GANs architecture is a style-based one. It was shown that alteration of generator architecture so that latent codes are provided in adaptive instance normalization blocks instead of the first convolutional layer leads to significant improvements in the quality of generated images as well as increased latent space disentanglement. In this work, we study the impact of quantization on style-based generator characteristics.


\subsection{Quantization of Generative Adversarial Networks}
There have been a few works investigating the quantization of GANs. Wang et al. \cite{wang2019qgan} utilized the expectation-maximization algorithm in order to quantize weights to a non-uniform grid of values while keeping activations unquantized. Despite promising results, the method under consideration cannot be directly used to reduce latency and perform computations in low bitwidth arithmetic; however, one still might find it useful for weights' compression. Wan et al. \cite{wan2020deep} approached the problem of quantization of deep generative models via a learnable non-uniform quantization scheme. Although it is theoretically possible to employ this method for low bitwidth inference in generative models, the non-uniform scheme utilized complicates deployment of this framework on edge devices.  Perhaps, the most relevant method was described in \cite{wang2020gan}. The authors applied uniform quantization to both weights and activations, combining quantization with pruning and knowledge distillation in a unified optimization framework. However, the paper is mainly concerned with compression techniques in general; thus, it misses some important insights about GANs quantization. For instance, the authors considered only 8-bit quantization of fully-convolutional architectures. Moreover, they fixed quantization parameters prior to training, while common practice \cite{esser2019learned} and our experiments show that it is beneficial to tune quantization parameters jointly with weights.
  %  \printbibliography
        
\end{document}

==> contribution.tex <==
%\documentclass[aa.tex]{subfiles}

\begin{document}


\end{document}
